FlowMind: Execute-Summarize for Structured Workflow Generation from LLM Reasoning

LLMs can solve complex tasks through reasoning and tool use, but accurately translating these solutions into structured workflows remains challenging. We model workflows as sequences of tool use and reformulate the problem as designing a mechanism that can both solve tasks and reliably construct workflows. Prior approaches that build workflows during execution often suffer from inaccuracies due to interference between the two processes. We propose an Execute-Summarize(ES) framework that decouples task execution from workflow construction: the model first completes the task using available tools, then independently reconstructs a structured workflow from execution traces. This separation improves workflow accuracy and robustness. We introduce FlowBench and show through extensive experiments that our approach outperforms existing methods, providing a reliable paradigm for grounding free-form LLM reasoning into structured workflows.

==> prompts/execute_summarize_context.tex <==
% execute_summarize_context.tex - Execute-Summarize策略：Summarize阶段上下文
% 源文件: agent_flow/orchestrator/execute_summarize/execute_summarize_orchestrator.py:306-344

\begin{table*}[t]
\centering
\scriptsize
\renewcommand\arraystretch{1.0}

\begin{tabular}{p{0.95\linewidth}}
\toprule[1.5pt]
\textbf{User Message Template: Summarize Stage - Text Summarization} \\
\midrule[1pt]

\textbf{Implementation:} Text Summarization reuses the ReAct or Plan-and-Execute system prompts (depending on configuration). This template formats the execution results as the user message input to the Summarize stage. \\
\\
\textbf{Strategy Options:} \\
\hspace*{1em}$\bullet$ \texttt{REACT}: Uses ReAct system prompt (Table~\ref{tab:react_system_prompt}) \\
\hspace*{1em}$\bullet$ \texttt{PLAN\_AND\_EXECUTE}: Uses Plan-and-Execute prompts (Tables~\ref{tab:plan_execute_planning_prompt}, \ref{tab:plan_execute_execution_prompt}) \\
\midrule

\textbf{Context Template (Injected as User Message):} \\
\texttt{\#\# Execution Results Context} \\
\\
\texttt{The following execution tasks have been completed. Use their results to fulfill the} \\
\texttt{summarization request.} \\
\\
\texttt{\{execution\_context\}} \\
\\
\texttt{\#\# Summarization Task} \\
\\
\texttt{\{summarize\_query\}} \\
\midrule

\textbf{Execution Context Format (per task):} \\
\texttt{\#\#\# Execution Task \{i\}: \{task\_id\}} \\
\texttt{**Query**: \{query\}} \\
\texttt{**Status**: $\checkmark$ Success / $\times$ Failed} \\
\texttt{**Result**: \{final\_answer\}} \\
\\
\texttt{**Execution Steps**:} \\
\texttt{- Step 1: `\{action\}` $\rightarrow$ \{observation\_summary\}} \\
\texttt{- Step 2: `\{action\}` $\rightarrow$ \{observation\_summary\}} \\
\texttt{...} \\
\bottomrule[1.5pt]
\end{tabular}%
\caption{Text Summarization context template for Summarize stage. The system prompt is determined by strategy (ReAct or Plan-and-Execute), while this template formats execution results as the user message input.}
\label{tab:execute_summarize_context}
\end{table*}

